W+jets, Z+jets, multijets and new physics searches

W+jets, Z+jets and QCD multijet production processes at hadron colliders are backgrounds to many searches for physics beyond the Standard Model which involve leptons and missing energy in the final state. We review the current theoretical and experimental status of these processes at the LHC. Furthermore, we discuss several methods that allow for reliable predictions for these processes in the context of new-physics searches.

==> Makefile <==
#-----------------------------------------------------
# This is a platform-independent Makefile to generate 
# dvi, ps and pdf files including Feynman Graphs using 
# FeynMP from the TeX source file MAIN_SRC. 
# The pdf filename is chosen via MAIN_PDF. 
#-----------------------------------------------------

MAIN_SRC = eps_proceedings

ARCHFLG  = $(shell if test `uname -s` == "Darwin"; then echo "preview"; \
	else echo "ghostview"; fi) 

MAIN:
		pdflatex $(MAIN_SRC).tex
		pdflatex $(MAIN_SRC).tex
		pdflatex $(MAIN_SRC).tex

preview:
	 	$(MAKE)
		open -a Preview $(MAIN_SRC).pdf

ghostview: 
	 	$(MAKE)
		gv -antialias $(MAIN_SRC).pdf

gv:
		$(MAKE) $(ARCHFLG)

feyn:


submit:
		tar czvf $(MAIN_SRC).tar.gz *.tex *.sty PoS* figures

tar:
		tar czvf $(MAIN_SRC).tar.gz *.tex *.sty Makefile PoS* figures

clean:
		rm -f *.log *.1 *.t1 $(MAIN_SRC).pdf *.aux *.dvi *~
		rm -f *.toc *.lof $(MAIN_SRC).tar.gz *.end *.pdfsync *.gz
